Interpretable Explanations of Black Boxes by Meaningful Perturbation

As machine learning algorithms are increasingly applied to high impact yet high risk tasks, such as medical diagnosis or autonomous driving, it is critical that researchers can explain how such algorithms arrived at their predictions. In recent years, a number of image saliency methods have been developed to summarize where highly complex neural networks "look" in an image for evidence for their predictions. However, these techniques are limited by their heuristic nature and architectural constraints. In this paper, we make two main contributions: First, we propose a general framework for learning different kinds of explanations for any black box algorithm. Second, we specialise the framework to find the part of an image most responsible for a classifier decision. Unlike previous works, our method is model-agnostic and testable because it is grounded in explicit and interpretable image perturbations.

==> old.tex <==
\newpage\appendix\section{Old text}

Answering the ``what'' question means describing the properties of the mapping $f$. For example, a classifier $f$ is often characterized in terms of its expected error rate. Other characterizations include: whether $f$ is invariant with a viewpoint change, if there are intra-class variations of the object that may confuse $f$, if $f$ recognizes the object by using contextual cues, and so on. Answering the ``how'' question means clarifying which computational mechanisms are used by $f$ in order to achieve such properties.

While the discussion has so far been informal, the next section attempts to formalize these concepts, focusing on the ``what'' question.

\subsection{Explaining what a predictor does}

An explanation of the predictor map $f:\mathcal{X}\rightarrow\mathcal{Y}$ is a succinct and meaningful characterization of some of its properties. For the a binary classifier, the most obvious property is to be correct. Formally, if $\mathcal{X}_+$ is the subset of images contain the object and $\mathcal{X}_-$ is its complement, correctness is given by the property:
\[
\forall x\in\mathcal{X}:\quad
e_1(x) = [f(x) = 1 \Leftrightarrow x \in \mathcal{X}_+].
\]
Another property is that ``$f$ is invariant to rotations of the image'', i.e.\
\[
  \forall x\in\mathcal{X},\ \theta\in[0,2\pi):\quad
  e_2(x,\theta) = [f(x) = f(R_\theta[x])],
\]
where $R_\theta$ rotates an image by the angle $\theta$.

Since predictors are rarely perfect, correct classification, invariance, or any other property may not be strictly satisfied; still, such explanations may still be useful if they apply with sufficiently large probabilities $P[e_1(x)]$, $P[e_2(x,\theta)]$. Note that computing such probabilities requires defining background probabilities $p(x)$ over images and/or over parameters such as rotations $\theta$.

Explanations should be informative. There are many uninformative true statements about $f$. For example, $e_3(x) = [|f(x)| \leq 1]$ is trivially satisfied by a binary classifier. Intuitively, a non-trivial explanation is one that applies to a small number of mappings $\mathcal{X}\rightarrow\mathcal{Y}$ and therefore distinguishes $f$ from other possible mappings. Making a quantitative theory out of this intuition is beyond the scope of this work.

Explanations may be expressed in terms of logical statements as done in the examples above, but this is not necessarily the case. More in general, an explanation may be built as an interpretable approximation of the predictor $f$, possibly valid only locally, in the vicinity $\mathcal{N}(x_0)$ of some point $x_0$. For instance:
\[
   \forall x \in \mathcal{N}(x_0):
   \quad
   e_3(x) = [ \| f(x) - f_e(x) \|^2 \leq \tau ]
\]
where $f_e(x)$ is a mapping that we understand. For instance, if $f:\mathbb{R}^D \rightarrow \mathbb{R}$ is an image and $f(x) \in \mathbb{R}$ is the score computed by a convolutional neural network, then the notion of \emph{network saliency} of~\cite{simonyan14deep}
\[
    f_e(x) = \langle \nabla f(x_0), x-x_0\rangle + f(x_0)
\]
is a local linear approximation of the classifier $f$ at image $x_0$. Note that~\cite{simonyan14deep} interpret $\nabla f(x)$ as a saliency measure; here, instead, the same gradient is used to define an approximation of the predictor $f$ that explains its structure locally. The latter use of the predictor gradient is due to~\cite{turner15a-model}. In the same paper, the authors suggests that, for other typologies of data for which individual dimensions of $x$ have a meaning, the approximating predictor $f_e$ may be expressed as a small decision tree or another simple interpretable rule. TODO: Find more references to this concept.
 
Interpretability is an important property of explanations since the main motivation for constructing them is to understand a predictor. For example, the gradient $\nabla f(x_0)$ can be displayed as an image to illustrate intuitively what changes to the image $x_0$ result in a change of the classifier output, and which ones do not. Explanations such as correctness and invariance use notions such as image class or image rotation that are also intuitive and interpretable.

In all examples above, explanations are interpretable rules that make predictions on the output of the mapping $f$. We readily distinguish two types of such predictors:
\begin{itemize}
\item {Absolute predictions} such as correctness expect the mapping $f$ to attain specific values at specific points in the domain.
\item {Relative predictions} such as invariance expect the value $f(x)$ to be related to the value $f(x')$ where points $x'$ and $x$ are related in some way. One can have equivariance relations of the type $f(gx)=gf(x)$, where a certain transformation $g$ acts on both input and output spaces, and invariance $f(gx)=f(x)$ as a special case.
\end{itemize}

\subsection{Invariance}

Most predictors are deemed to be \emph{invariant} to certain variability factors affecting the data. For example, in image recognition, a predictor $f$ is often \emph{translation invariant}, in the sense that $f(x) \approx f(\mathcal{L}_t(x))$ where $\mathcal{L}_t$ is an operator that translates the image $x$ by an amount $t$. More in general, if $g : \mathbb{R}^2 \rightarrow \mathbb{R}^2$ is a bijection such as a rotation, a scaling, or a more general affine distortion of the plane, then one may check for invariances $\forall x \in X: f(x) \approx f(gx)$.

This definition of invariance, which involves only mathematical concepts, is not very useful in practice. Note that a function which is invariant to warps $g$ and $g'$ must be invariant to to $g'g$ as well (because $f((g'g)x) = f(g'(gx)) = f(gx) = f(x)$). Thus invariance to image warps, as well as any other class of composable transformations, is only possible for entire entire subgroups $G$ of the transformation group $\mathbb{R}^2 \rightarrow \mathbb{R}^2$. Transformation groups are generally very large. The most general group $\mathcal{G}(\mathbb{R}^2)$ contains all invertible maps $\mathbb{R}^2 \rightarrow \mathbb{R}^2$ (think of these as permutations of all points of the plane), and usual restrictions consider the subgroups of continuous $\mathcal{C}^0(\mathbb{R}^2)$ or $k$-times differentiable $\mathcal{C}^k(\mathbb{R}^2)$ (diffeomorphisms) maps. Other common restrictions consider Lie groups such as affine transformations, dilations, similarities, isometries (Euclidean transformations), translations, etc. Even if we fix a single transformation, say a translation $g$ by two pixels to the right, the smallest group containing $g$, i.e.\ the cyclic group generated by $g$, contains all iterated translations $g^n$.

Since the image $x$ is in practice finite (in resolution and extent), any of such group is clearly too much: a predictor cannot be invariant to a translation that moves the object out of the image, or to a scaling that makes it smaller than a single pixel. Thus, such notions are useful only in an idealized sense, but are not directly applicable to actual predictors.

In order to make invariance a more useful concept, one needs to add to mathematical constructions a number of statistical assumptions. For example, note that, if $g$ is a transformation of the plane, $gx$ is undefined if $x$ is a digital image, which has a finite resolution and extent. The finite resolution of $x$ is usually addressed by making the \emph{statistical} assumption that $x$ is the sampled version of a band-limited image, so that one can use interpolation. The finite extent of the image is addressed by continuing the image by using padding or reflection.

We may ask, are such assumptions reasonable? One approach to answer this question, which will be considered in more detail later, is to realize that transformations of the image arise as proxies to transformations occurring in the physical world; for example, a visual classifier should be invariant to motions of the 3D camera, which can sometimes be approximated by certain image transformations. In this sense, the assumptions above are not particularly good: moving a physical camera translation will reveal new information (by unoccluding portions of the scene or by revealing small details) which cannot, and in fact is not, recovered by emulating transformations in image space.

One can define invariance in very general terms by considering any partition of the set of images $X$, which in turns induces an equivalence relation $x \sim x'$ between images. The mapping $f$ is invariant with $\sim$ when
\[
     x\sim x' \quad\Rightarrow\quad f(x) = f(x').
\]

\subsection{The decision support of image predictors}

We now focus our attention on predictors $f :\mathcal{X}\rightarrow\mathcal{Y}$ operating on the set $X = \mathbb{R}^{H\times W \times C}$ of $H \times W$ digital images with $C$ color channels. Deep convolutional neural networks are the most important family of such predictors.

Compared to a general predictor, one obvious property of an image predictor is the fact that the input data has a \emph{spatial structure}. Most visual object are local phenomena, in the sense that their projection on the image has a finite extent. One natural question is whether a predictor focuses on the extent of such objects, or whether it uses contextual cues in the image.

As noted above, given an example image $x_0$, one may study the \emph{sensitivity} of the predictor function $f(x)$ to local changes in the input $x_0$.




\begin{itemize}
\item $S(\Omega) = E[|f(x_0 + \eta_\Omega) - f(x_0)|]$.
\item $\operatorname{supp}_\tau f = \cup_{S(\Omega) \geq \tau} \Omega$.
\end{itemize}




\begin{itemize}
\item Definition of saliency/what is a good explanation? How do you measure the quality of an explanation? Why do we want to explain what the networks are doing/learning? (i.e. correlation not causation, human examples; systematic bias -- cardigan example)
\item Single-shot change vs summary of multiple changes
\item Optimization vs bulk change (box occluder)
\item Meaning of editing operation
\item Deletion vs preservation of object
\item Mask regularization
\item Eliminate mask-introduced artifacts (i.e. regularize so that the network prediction is well-distributed across classes)
\end{itemize}

\section{Unraveling black-box decisions}

Let $x \in \mathcal{X}$ denote an image. In general, a grayscale image is a function $x : D \rightarrow \mathbb{R}$ where $D = \{1,2,\dots,N\}^2$ is a two-dimensional $N\times N$ lattice. It is also possible to consider 1D images (time signals) as well.

We are given a black-box binary classifier function $f : \mathcal{X} \rightarrow \{+1,-1\}$ separating the set of images in positive and negative. Usually the positive class, i.e.\ the subset of images that are assigned positive label, is usually much smaller than the negative one.

Given a positive image $x$, such that $f(x)=+1$, we would like to find an \emph{explanation} of why the classifier assigns a positive label to $x$. Defining explanation is challenging. We consider below several approaches below.

\subsection{Explanation as simplified interpretable classification rules}

We consider first the approach of~\cite{turner15a-model}. For them, an explanation $e$ of a binary classifier $f$ is also a  binary classifier $e : \mathcal{X}\rightarrow\{+1,-1\}$, but with a particularly simple and interpretable structure (e.g.\ a conjunction of a few binary tests). The collection of explanation functions $e$ is denoted $\mathcal{E}$. Each explanation is regarded as an ``approximation'' $e \approx f$ of the black-box binary classifier $f$ that one wants to understand. The quality of the approximation is measured based on how well the responses of $e$ and $f$ agree \emph{on average} with respect to a certain background data distribution $p(x)$. The agreement can be measured, for example, as the mutual information $I(e,f)$. In order to explain a \emph{particular} decision $f(x)=+1$ for a certain data point $x$, one looks for the explanation $e\in\mathcal{E}$ that is the best approximation to $f$ in general while matching the output of $f$ at $x$ (i.e.\ $e(x) = f(x) = +1$). Hence, the explanation is a semi-local interpretable approximation of the classifier.

Note that, in this framework but likely in general, while one seeks an explanation for a particular data point $x$, the latter must somehow reflect the response of the classifier $f$ on other points as well. In the formulation above, for example, it is trivial to construct a simple rule that matches any data point $x$ (e.g.\ $e(z) = \delta_{\{z=x\}}$); instead, a useful explanation must be interpretable while at the same time being general, i.e.\ predictive of as many other decisions $f(z)=e(z)$ as possible.

This formulation requires a mechanism for generating interpretable explanations. The authors of~\cite{turner15a-model} propose to use a small decision tree or conjunction of simple tests, which in turn must be based on interpretable data statistics. This idea is of difficult applicability to images. However,~\cite{turner15a-model} demonstrates a simple image-based experiment. There, explanations $e(x;w,b) = \sign \langle w,x \rangle +b$ are eigenfaces $w \in \{w_1,\dots,w_n\}$. In this framework, a face classification $f(x)=1$ is explained by choosing $i \in \{1,\dots,n\}$ and $b \in \mathbb{R}$ such that
\[
	\max_{k,b} I(e(z;w_k,b),f(z))_{z\sim p}
    \quad
    \text{such that\ }  e(x;w_k,b) = +1
\]
Such explanations are in effect linear classifiers. They are interpretable in the sense that they produce pixel weight masks or heatmaps. This has a connection with the standard notion of network saliency:
\[
   f(z) \approx e(z;w,b) = \langle w,z \rangle + b,
\]
where
\[
   w = \frac{df(x)}{dx},
   \qquad b = f(x) - \langle w, x \rangle.
\]
Note that $w$ is also a local linear approximation of the classifier $f(x)$. Generalizing these considerations, we may think of these as \emph{explanation via local classifier simplification}.

\subsection{Explanation support} 

With images and similar distributed signals $x : D \rightarrow \mathbb{R}$,  often only a subset $\Omega \subset D$ of the pixels should be relevant for a given decision $f(x)=1$. A typical example is object recognition: only foreground pixels, i.e.\ the pixels belonging to the object, should be directly responsible for the decision, whereas background pixels should provide at most indirect evidence.

The question, then, is how one can identify which pixels $x$ are ``directly responsible'' for a given decision. This apparently innocuous question is fraught with difficulties.

The starting point is simple enough: if only pixels $\Omega$ are responsible for a decision, then: 1) deleting the pixels in $D / \Omega$ should not change the decision while 2) deleting the pixels in $\Omega$ should change the decision. However:

\begin{itemize}
\item ``Deleting'' pixels is not clearly defined. We may delete them by setting them to zero, to noise, to some other image, by smooth infilling the hole, and so on.

\item Informative pixels are often at the boundary of the object as the silhouette is often very informative. Since the silhouette is recognized by contrasting foreground and background pixels, clearly both pixel types are responsible for the recognition of the object. For example, consider a black disk on a white background. Neither the white or black infills are very informative; rather, the shape is recognized by observing the transition from white to black.

\item Deleting a small subset of strategically deleted pixels may be enough to make the object invisible for the. For instance, one may just delete the boundary and preserve the interior, or perhaps delete every other row. While not all object pixels are deleted, the network does fail to recognized the object.

\item Conversely, conserving a subset of strategically-placed pixels may be enough to allow the network to still recognize the object. For example, preserving the object silhouette when deleting only the interior, or preserving only a distinctive part of the object while deleting the rest.

\item Deletion, just like any other image editing operation, may introduce artifacts. E.g. an image of an object can be carved out by deleting bits of a uniform background.  More subtle artifact in the way neural networks parse iamges may be triggered by highly-specialized (overfitted) forms of image editing driven for example by gradient descent.
\end{itemize}

\begin{example}
Let's consider a 1D function $x: [0,1] \rightarrow \mathbb{R}$. Consider a classifier
$$
f(x) = 
\begin{cases}
1, & \exists u\in [0,1] : x(u) > 0, \\
0, & \text{otherwise}.
\end{cases}
$$
I.e.\ the classifier fires if the ``image'' $x$ has at least one pixel $u$ such that $x(u) > 0$. Now we see that \emph{any} such pixel is a support for the decision $f(x)=+1$, in the sense that we can change the value of any other pixel obtaining a second image $x'$ such that $f(x')=+1$ as well. However, a better explanation is probably inclusive of all such sufficient pixels.
\end{example}

\paragraph{Multi-category classification}
In reality, most black-box algorithms are not solving simple binary classification problems. In the multi-category classification setting (i.e. ImageNet classification), there may be competition between categories.
\begin{example}
Consider a multi-category classifier that classifies a shape as one of three possibilities: a triangle, a square, or a circle.
\end{example}



==> scratch.tex <==
\section{Scratch}
\begin{table}
\begin{center}
\begin{tabular}{|r|c|c|c|c|c|c|c|c|}
\hline
& 
%\footnotesize{Grad~\cite{simonyan14deep}} &
%\footnotesize{Guid~\cite{springenberg2014striving,mahendran2016salient}} & 
%\footnotesize{Exc~\cite{zhang2016top}} & 
%\footnotesize{Cont Exc${}^\dagger$~\cite{zhang2016top}} & 
%\footnotesize{Feedb${}^\dagger$~\cite{cao2015look}} & 
%\footnotesize{LRP${}^\dagger$~\cite{bach2015pixel}} & 
%\footnotesize{CAM${}^\dagger$~\cite{zhou2016learning}}& 
%\footnotesize{Mask} \\

\footnotesize{~\cite{simonyan14deep}} & \footnotesize{~\cite{springenberg2014striving,mahendran2016salient}} & 
\footnotesize{~\cite{zhang2016top}} & 
\footnotesize{C-~\cite{zhang2016top}} & 
\footnotesize{~\cite{cao2015look}} & 
\footnotesize{~\cite{bach2015pixel}} & 
\footnotesize{~\cite{zhou2016learning}}& 
\footnotesize{Mask} \\
\hline\hline
\footnotesize{Value-$\alpha$*} & \footnotesize{0.25} & \footnotesize{0.05} & \footnotesize{0.15} & \footnotesize{---}  & \footnotesize{---}  & \footnotesize{---}  & \footnotesize{---}  &\footnotesize{0.10} \\
\footnotesize{Err (\%)} & \footnotesize{47.0} & \footnotesize{51.2} & \footnotesize{47.1} & \footnotesize{---}  & \footnotesize{---}  & \footnotesize{---} & \footnotesize{---}  &\footnotesize{45.1} \\
\hline\hline
\footnotesize{Energy-$\alpha$*} & \footnotesize{0.10} & \footnotesize{0.30} & \footnotesize{0.60} & \footnotesize{---}  & \footnotesize{0.95} & \footnotesize{---}  & \footnotesize{---}  & \footnotesize{0.95} \\
\footnotesize{Err (\%)} & \footnotesize{44.9} & \footnotesize{48.0} & \footnotesize{39.9} & \footnotesize{---}  & \footnotesize{38.8${}^\dagger$} & \footnotesize{---}  & \footnotesize{---}  & \footnotesize{44.3} \\
\hline\hline
\footnotesize{Mean-$\alpha$*} & \footnotesize{5.0} & \footnotesize{4.5} & \footnotesize{1.5} & \footnotesize{0.0} & \footnotesize{---}  & \footnotesize{1.0} & \footnotesize{1.0} & \footnotesize{0.5} \\
\footnotesize{Err (\%)} & \footnotesize{41.7${}^\mathsection$} & \footnotesize{42.0${}^\mathsection$} & \footnotesize{39.0${}^\mathsection$} & \footnotesize{57.0${}^\dagger$} & \footnotesize{---}  & \footnotesize{57.8${}^\dagger$} & \footnotesize{48.1${}^\dagger$} & \footnotesize{44.3}\\
\hline
\end{tabular}
\end{center}
\caption{Optimal alpha thresholds and error rates from the weak localization task on the ImageNet validation set using saliency heatmaps to generate bounding boxes. *Feedback error rate are taken from~\cite{cao2015look}; contrastive excitation backprop, LRP and CAM error rates are taken from~\cite{zhang2016top}. ${}^\mathsection$Using public code provided in~\cite{zhang2016top}, we recalculated these error rates, which are within $0.4\%$ of the originally reported rates.}
\label{t:localization}
\end{table}


Generalizing these examples, an explanation is a rule that predicts the response of the map $f$ to certain inputs. Rules with a strong explanatory power are simple, general, interpretable, and informative. For example, a tautology such as ``the output of the binary classifier $f$ is either $-1$ or $+1$'' is uninformative. Using $f$ as a rule to predict its own values is equally useless as it is not simple nor interpretable. Discrimination is interpretable but only mildly informative because we would expect a classifier to be correct for its task. The discrimination rule above is complex as it requires to define the set $\mathcal{X}_+ \subset \mathcal{X}$ of images containing the target class. Importantly, while the set $\mathcal{X}_+$ can be very complex, it is defined independently of $f$ \emph{a-priori}. Rotation invariance is, by comparison, a simpler rule.

Since the learned map $f$ is usually imperfect, it is unreasonable to expect explanatory rules to be strictly correct. To allow some slack, we can allow the rule to work correctly for most inputs, or with a certain degree of accuracy, or both. For example, rules such as discrimination can be expressed by predicates
\begin{align*}
Q_1(x;f)    &= \lp x \in\mathcal{X}_c  \Leftrightarrow  f(x) = +1 \rp, \\
Q_2(x,x';f) &= \lp x \sim_\text{rot} x' \Rightarrow f(x) = f(x') \rp,
\end{align*}
where $x \sim_\text{rot} x'$ means that images $x$ and $x'$ are related by a rotation. Given a distribution $p(x)$ over images, the \emph{faithfulness} of the explanations can be measured as the probabilities $P[Q_1(x;f)]$ and $P[Q_2(x,x';f)|x \sim x']$ that the predicates are true. Predictions need not to be binary either; for example, if the output of $f$ is continuous, then faithfulness of rotation invariance could be measured by the expected squared residual $E[(f(x) - f(x'))^2|x \sim x']$ (where lower means more faithful).

\subsubsection{Other explanation types}\label{s:types}

So far, we have considered (semi-)categorical explanations, but many other interesting cases are possible. For instance, if $f$ is a regressor and the output space $\mathcal{Y}\subset\mathcal{R}^d$ is continuous, categorical predictions are not useful. Instead, explanations can also perform predictions in the same space $\mathcal{Y}$ and their accuracy can be measured by suitable error terms other than the boolean prediction error used above.

Here is a particularly relevant example. Consider a neural network $f$ producing a confidence score in $\mathcal{R}$. Then we can \emph{explain $f$ locally} by means of the function derivatives:
\[
      f(x + \delta_x) \approx f(x) + \langle \nabla f(x),\delta_x\rangle.
\]
The explanation is the gradient $\nabla f(x)$ which describes how the map $f$ behaves locally. It corresponds to the \emph{network saliency} of~\cite{simonyan14deep} and, as suggested by those authors, it can be visualized as an \emph{image}.

\paragraph{Derivation of saliency in this framework.} Here is how the concept of network saliency emerges in our framework. To express the fact that we are seeking a local approximation, we consider a \emph{distribution} $p(x|x_0)$ of images $x$ around a reference image $x_0$. We then approximate $f(x)$ by means of a linear function $\langle w, x-x_0\rangle$ as follows:
\[
 \min_w \lambda |w|^2 +
 E_{p(x|x_0)}
 \left[
 (f(x) - f(x_0) - \langle w, x-x_0 \rangle)^2
 \right]
\]
We see that the optimum is given by zeroing the gradient w.r.t.\ $w$:
\[
0=
\lambda w
+
E
 \left[
 (x-x_0) (f(x) - f(x_0) - \langle w, x-x_0 \rangle)
 \right]
\]
Hence
\[
w = 
\left\{\lambda I + E[(x-x_0)(x-x_0)^\top]\right\}^{-1}
E[(x-x_0) (f(x) - f(x_0))].
\]
Assume that $p(x|x_0)$ is a Gaussian centred on $x_0$ and with variance $\Sigma_x$. Assume also that $f(x)-f(x_0)= \langle \nabla f(x_0), x-x_0\rangle$. Then
\[
w = (\lambda I + \Sigma_x)^{-1}\Sigma_x \nabla f(x_0).
\]
If the variance is isotropic, then this is simply a scaled version of Simonyan et al.\ saliency.

\paragraph{Generalization 1 (bad?).} Consider now a distrubution over $x$ obtained by applying a translational jitter $\delta_u \sim \mathcal{N}(0,\sigma_u^2 I)$ to $x_0$:
\[
 x(u) = x_0(u) + \langle \nabla x_{0}(u), \delta_u \rangle
\]
\[
 E[(x(u)-x_0(u))(x(v) - x_0(v))]
 =
\sigma_u^2 \langle \nabla x_{0}(u), \nabla x_{0}(v) \rangle
\]
Hence in this case $\Sigma_x$ has a particularly simple form. Let $\nabla x$ be the $2 \times N^2$ matrix of the gradients of the image at each pixel; then:
\[
 \Sigma_x = \sigma_u^2 (\nabla x)^\top(\nabla x)
 =
 \sigma_u^2 U^\top S U
\]
where $U$ is a $2\times N^2$ orthonormal matrix ($U U^\top = I_{2\times 2}$). For the majority of images, we can assume that $S= s^2I$ is diagonal, so that
\[
 w = \sigma_u^2 s^2(\lambda I + \sigma_u^2 s^2 U^\top U)^{-1} U^\top U \nabla f(x_0).
\]

\paragraph{Explaining a linear predictor.} A linear predictor is a simple rule $f(x) = \langle w, x \rangle$. The rule itself is mechanically straightforward: the prediction is the sum the weighted data components $w_ix_i$. Applying the saliency framework discussed above, the \emph{explanation} of the classifier is simply $w$ itself. This explanation is also independent of the particular input $x$. This is because, since the predictor is linear, any change $\delta_x$ to the pattern results in the same variation $\langle w, \delta_x \rangle$ of the prediction score regardless of the specific value of $x$.

